BOP Challenge 2022 on Detection, Segmentation and Pose Estimation of Specific Rigid Objects

We present the evaluation methodology, datasets and results of the BOP Challenge 2022, the fourth in a series of public competitions organized with the goal to capture the status quo in the field of 6D object pose estimation from an RGB/RGB-D image. In 2022, we witnessed another significant improvement in the pose estimation accuracy -- the state of the art, which was 56.9 AR$_C$ in 2019 (Vidal et al.) and 69.8 AR$_C$ in 2020 (CosyPose), moved to new heights of 83.7 AR$_C$ (GDRNPP). Out of 49 pose estimation methods evaluated since 2019, the top 18 are from 2022. Methods based on point pair features, which were introduced in 2010 and achieved competitive results even in 2020, are now clearly outperformed by deep learning methods. The synthetic-to-real domain gap was again significantly reduced, with 82.7 AR$_C$ achieved by GDRNPP trained only on synthetic images from BlenderProc. The fastest variant of GDRNPP reached 80.5 AR$_C$ with an average time per image of 0.23s. Since most of the recent methods for 6D object pose estimation begin by detecting/segmenting objects, we also started evaluating 2D object detection and segmentation performance based on the COCO metrics. Compared to the Mask R-CNN results from CosyPose in 2020, detection improved from 60.3 to 77.3 AP$_C$ and segmentation from 40.5 to 58.7 AP$_C$. The online evaluation system stays open and is available at: \href{http://bop.felk.cvut.cz/}{bop.felk.cvut.cz}.

==> fig_pbr_examples.tex <==
\begin{figure}[t!]
\begin{center}

\begingroup
\renewcommand{\arraystretch}{0.9}

\begin{tabular}{ @{}c@{ } @{}c@{ } @{}c@{ }}

\includegraphics[width=0.333\columnwidth]{img/bop20_pbr_ycbv_01.jpg} &
\includegraphics[width=0.333\columnwidth]{img/bop20_pbr_ycbv_03.jpg} &
\includegraphics[width=0.333\columnwidth]{img/bop20_pbr_lm_06.jpg}  \\

\includegraphics[width=0.333\columnwidth]{img/bop20_pbr_icbin_01.jpg} &
\includegraphics[width=0.333\columnwidth]{img/bop20_pbr_tless_01.jpg} &
\includegraphics[width=0.333\columnwidth]{img/bop20_pbr_itodd_02.jpg} \\

\end{tabular}
\endgroup

\caption{\label{fig:pbr_examples} \textbf{Synthetic training images.} Participants were provided 350K photorealistic training images procedurally generated and rendered using BlenderProc~\cite{denninger2019blenderproc,denninger2020blenderproc}. 
}

\end{center}
\end{figure}


==> tab_cosypose_data.tex <==
\setlength{\tabcolsep}{5pt}
\begin{table}[t]
\centering

\begingroup
\footnotesize
\begin{center}
\begin{tabularx}{\textwidth}{ c c *{3}{Y} }
	\toprule
	Detection & Pose estim. & T-LESS & TUD-L & YCB-V \\
	\midrule
	PBR+Real & PBR+Real & 72.8 & 82.3 & 82.1 \\
	PBR & PBR & 64.0 & 68.5 & 57.4 \\
	PBR & Render\,\&\,paste v1 & 16.1 & 60.4 & 44.9 \\
	PBR & Render\,\&\,paste v2 & 60.0 & 58.9 & 58.5 \\
	Render\,\&\,paste v1 & Render\,\&\,paste v1 & 6.1 & 49.5 & 26.5 \\
	Render\,\&\,paste v2 & Render\,\&\,paste v2 & 45.3 & 42.4 & 25.7 \\
	\bottomrule
\end{tabularx}
\end{center}

\caption{\label{tab:cosy_data_res} \textbf{The effect of different training images}. The table shows the $\text{AR}_{\text{Core}}$ scores achieved by the CosyPose method~\cite{labbe2020cosypose} when different types of images were used for training its object detection (\ie Mask R-CNN~\cite{he2017mask}) and pose estimation stage.
The ``render\;\&\;paste v1'' images were obtained by OpenGL rendering of the 3D object models on random real photographs.
The ``render\;\&\;paste v2'' images were obtained similarly, but the CAD models of T-LESS objects were assigned a random surface texture instead of a random gray value, the background of most images was assigned a synthetic texture, and 1M instead of 50K images were generated.
Interestingly, the increased photorealism brought by the PBR images yields noticeable improvements despite the strong data augmentation applied by CosyPose to the training images.
\vspace{5.3ex}
}
\endgroup

\end{table}

